Is Graph Convolution Always Beneficial For Every Feature?

Graph Neural Networks (GNNs) have demonstrated strong capabilities in processing structured data. While traditional GNNs typically treat each feature dimension equally during graph convolution, we raise an important question: Is the graph convolution operation equally beneficial for each feature? If not, the convolution operation on certain feature dimensions can possibly lead to harmful effects, even worse than the convolution-free models. In prior studies, to assess the impacts of graph convolution on features, people proposed metrics based on feature homophily to measure feature consistency with the graph topology. However, these metrics have shown unsatisfactory alignment with GNN performance and have not been effectively employed to guide feature selection in GNNs. To address these limitations, we introduce a novel metric, Topological Feature Informativeness (TFI), to distinguish between GNN-favored and GNN-disfavored features, where its effectiveness is validated through both theoretical analysis and empirical observations. Based on TFI, we propose a simple yet effective Graph Feature Selection (GFS) method, which processes GNN-favored and GNN-disfavored features separately, using GNNs and non-GNN models. Compared to original GNNs, GFS significantly improves the extraction of useful topological information from each feature with comparable computational costs. Extensive experiments show that after applying GFS to 8 baseline and state-of-the-art (SOTA) GNN architectures across 10 datasets, 83.75% of the GFS-augmented cases show significant performance boosts. Furthermore, our proposed TFI metric outperforms other feature selection methods. These results validate the effectiveness of both GFS and TFI. Additionally, we demonstrate that GFS's improvements are robust to hyperparameter tuning, highlighting its potential as a universal method for enhancing various GNN architectures.

==> sections/planning.tex <==
\section{Planning}

\begin{itemize}
    \item Main table Method best 09-10
    \item Theory Proof 09-10, CSBM, MLP GCN perferred features; MI is better.
    \item Analysis 09-10
    \item Paper writing 09-15
    \item Revision 09-20
    \item 
\end{itemize}

\begin{itemize}
    % \item Run Empirical Experiments

    % 1. Get other feature homophily values (agg\_homo\_soft, agg\_homo\_hard, node\_hom\_generalized, cls\_ctrl\_feat\_homo, attr\_homo, localsim\_cos\_homo, localsim\_euc\_homo) on commonly use graphs (minesweeper, roman-empire, amazon-ratings, tolokers, questions, squirrel-filtered, chameleon-filtered, actor, texas-4-classes, cornell, wisconsin, cora, citeseer, pubmed)\finish{80}

    % 2. Propose a new metric that can reflect GNNs performance. The correlation of our metric must outperform the other homophily baselines on most datasets in correlation.\finish{70}

    % 3. Detect graph-favored and graph-disfavored features using our metric. Show middle ratio is the best \finish{100}

    % \item Proposed Method \finish{80}

    % 1. Calculate MI on aggregated feature and labels (feature-wise) \finish{100}

    % 2. Feed graph-favored features to GNNs and graph-disfavored features to MLP as the backbone. \finish{100}

    % 3. Complexity analysis \finish{0}

    % \item Theoretical Proof 
    
    % 1. Prove our metric is related with GraphConv and feature homophily could fail. \finish{100}

    % 2. Prove our metric is the upper bound of GNNs-MLP \finish{100}

    \item Experiments

    1. Show our proposed method is better compared with other baselines\finish{100}. Add more GNN baselines\finish{30} 3h. Add tuning\finish{30} 1h.

    2. \finish{100} Ratio tuning

    3. \finish{50}. Comparison hom metrics 2h. Use other feature homophily to detect graph-favored/disfavored features, compare with ours 1h.

    4. \finish{100} Ablation; Swap these two features for GNN and MLP and see if performance drops.
    
    5. \finish{100} Accuracy change with bins of features on GCN and MLP 3h.

    6. \finish{0} Semi-supervision minor impact on acc 1h
    
    7. \finish{0} Our statistics-based method is better than optimization methods 5h.

    8*. \finish{0} exploring k-hop neighbors of TFI 1h.
    
    9*. \finish{0} insensitive to hyper-parameter tuning, overall improvement without tuning 0.5h.
    
    \item Paper Writing
    Abatract\finish{80}, Introduction, Related Work, Preliminary, New Feature Homophily Metric, Proposed Method, Experiments, Conclusion. Appendix
    
\end{itemize}

KTTRCDL note     % KTTRCDL note
    
Dataset: ["amazon-ratings", "minesweeper", "questions", "roman-empire", "tolokers"] appendix: ['squirrel-filtered', 'chameleon-filtered', 'actor', 'texas-4-classes', 'cornell', 'wisconsin', 'cora', 'citeseer', 'pubmed'] 

\textbf{TODO}: feature selection: ["mutual\_info\_classif", "cls\_ctrl\_feat\_homo", "attr\_homo", "node\_hom\_generalized", "localsim\_cos\_homo", "localsim\_euc\_homo", "agg\_homo\_soft"] \\
\textbf{Done}: ["mutual\_info\_classif", "cls\_ctrl\_feat\_homo", "attr\_homo", "node\_hom\_generalized"]

mutual information variant: ["mi\_agg", "mi\_aggego"] %为什么要这么做呢？因为如果直接检查原始的特征和标签的mi（互信息），反映不了GNN的性能，因为GNN包含了邻居信息。所以我们对所有特征做一次聚合操作，然后再与标签比较，这样可以很好地反映到底GNN为什么在这个特征上面好（因为拓扑信息已经被包括进去了）

TODO: model ["GCN-MLP", GAT, SGC, GraphSage, APPNP]

TODO: Tuning 
Layer [2,3]
hidden dim [128, 256, 512]
lr [1e-3, 1e-4, 1e-5] 
weight decay [1e-3, 3e-4, 1e-4, 3e-5, 1e-5]
dropout [0.2, 0.3, 0.4, 0.5, 0.6]

["amazon-ratings", "minesweeper", "questions", "roman-empire", "tolokers"] mi\_agg 
ratio
amazon-ratings: 0.6
minesweeper: 0.9
questions: 0.9
roman-empire: 0.2
tolokers: 0.7

\textbf{TODO}:
* main table \LaTeX print

* metrics localsim\_cos\_home localsim\_euc\_homo agg\_homo\_soft

* fix dataset statistics \LaTeX print

* ACM-GCN
